Parametric Fairness with Statistical Guarantees

Algorithmic fairness has gained prominence due to societal and regulatory concerns about biases in Machine Learning models. Common group fairness metrics like Equalized Odds for classification or Demographic Parity for both classification and regression are widely used and a host of computationally advantageous post-processing methods have been developed around them. However, these metrics often limit users from incorporating domain knowledge. Despite meeting traditional fairness criteria, they can obscure issues related to intersectional fairness and even replicate unwanted intra-group biases in the resulting fair solution. To avoid this narrow perspective, we extend the concept of Demographic Parity to incorporate distributional properties in the predictions, allowing expert knowledge to be used in the fair solution. We illustrate the use of this new metric through a practical example of wages, and develop a parametric method that efficiently addresses practical challenges like limited training data and constraints on total spending, offering a robust solution for real-life applications.

==> proofs_arxiv.tex <==
%\begin{document}
\onecolumn

\begin{center}
\bf{\Large Parametric Fairness with Statistical Guarantees: \\
Supplementary Materials}
\end{center}

\appendix

\section{Broader Impact}
 Our work is centered around fairness, which is a goal we sincerely believe all model should strive to achieve. Nevertheless, to ensure fairness in models, one needs to define unfairness as its counterpart. This naturally leads to a conundrum when performing research on the topic. On one hand, we would like our models to be fair, but to analyse the differences and show an improvement, we first need to create an unfair outcome. As has been shown in the past, simply ignoring the sensitive attributes does not solve the problem of bias in the data. Further, as more flexible methods make their way into practical applications, this issue is only bound to increase. Hence it is our conviction that estimating intentionally unfair models (by for example including sensitive variables explicitly in the training phase) is ethically justifiable if the goal is to provide a truly fair estimation. In that sense our work contributes to achieving fairness, and does not create new risks by itself. 

In our empirical application, we consider both data for wages and criminal justice. As has been discussed numerous times before in the media and academic research, there is a discrepancy between scores and predictions obtained for sensitive groups in these data sets. To avoid any misguided interpretation, we refrain from specifying the features directly, and merely use a subset of sensitive features to demonstrate the effectiveness of our method. Our goal here is to contribute to the body of research aiming to correct biases from arbitrary machine learning models and hence we put our focus on the metrics associated with this. In theory, we could use arbitrary data, but in the spirit of easier comparability, we opted to use well-known and publicly accessible data sets. We believe the safeguards taken and the use of the data in this context justify its use. 

\section{Proofs}

In this section, we gather the proofs of our results. Section~\ref{subappx:tech} covers essential fairness results in non-parametric fair regression. The proof for parametric fair predictors in the exact fairness framework is detailed in Section~\ref{subappx:main}. We also extend these results to approximate fairness in Section~\ref{subappx:approx} and discuss the theoretical properties of our estimation procedure in Section~\ref{subappx:cvg}.

\subsection{Fair Regression}\label{subappx:tech}

Recall that $g^*(\boldsymbol{X}, S) = \mathbb{E}[Y | \boldsymbol{X}, S]$ where we consider the general regression problems (can be extended to vector-valued problems)
\begin{equation*}\label{eq:RegGeneral}
   Y = g^{*}(\boldsymbol{X}, S) + \zeta \enspace,
\end{equation*}
with $\zeta\in\mathbb{R}$ a zero mean noise. The following lemma is adapted from \cite{gouic2020projection}. 

\begin{lem}[\cite{gouic2020projection}]\label{lem:ERisk}
    For a subclass of regressors $\mathcal{H}\subset\mathcal{G}$, if for any $h\in\mathcal{H}$ and $g\in\mathcal{G}$, where,
    $$
    \nu_{g|s} = \nu_{h|s} \quad \text{for all } s\in\mathcal{S}\enspace,
    $$
    we have $g\in\mathcal{H}$, then we can derive the associated excess-risk as,
    \begin{equation}
        \mathcal{E}(\mathcal{H}) = \inf_{h \in \mathcal{H}}\sum_{s\in\mathcal{S}}p_s \mathcal{W}_2^2\left(\nu_{g^*|s}, \nu_{h|s}\right)\enspace.
    \end{equation}
\end{lem}

%\begin{proof}
% From Pythagoras' Theorem we can derive directly:
%\begin{align*}
     %\mathbb{E}[\norm{\boldsymbol{Y}-g^*(\boldsymbol{X}, S)}^2] + \mathbb{E}[\norm{h(\boldsymbol{X}, S) - g^*(\boldsymbol{X}, S)}^2] = \mathbb{E}[\norm{\boldsymbol{Y} - h(\boldsymbol{X}, S)}^2]
%\end{align*}
%and therefore
%\begin{align*}
% \inf_{h \in \mathcal{H}} \mathbb{E}[\norm{Y - h(\boldsymbol{X}, S)}^2] - \mathbb{E}[\norm{Y - g^*(\boldsymbol{X}, S)}^2] =  \inf_{h \in \mathcal{H}} \mathbb{E}\big[\mathbb{E}[\norm{h(\boldsymbol{X}, S) - g^*(\boldsymbol{X}, S)}^2 | S]\big]
%\end{align*}
%From the definition of the Wasserstein distance we have that:
%\begin{align*}
%    \mathbb{E}[\norm{h(\boldsymbol{X}, S) - g^*(\boldsymbol{X}, S)}^2|S] \geq \mathbb{E}[\mathcal{W}_2^2(\nu_{g^*|S}, \nu_{h | S})]
%\end{align*}
%Finally, since Assumption~\ref{assu:general} holds,
%there also exists an optimal transport map $T_s:\mathbb{R}^L\to \mathbb{R}^L$ such that $T_s(g^*(\boldsymbol{X}, s)) \sim \nu_{h | s}$ and
%\begin{align*}
%     \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{h | s}) &= \mathbb{E}[\norm{T_s(g^*(\boldsymbol{X}, s)) - g^*(\boldsymbol{X}, s)}^2]\enspace.
%\end{align*}
%Since $g\in\mathcal{H}$ for any $(\nu_{g|s})_s = (\nu_{h|s})_s$ where $h\in\mathcal{H}$, it implies that 
%\begin{align*}
%    \mathbb{E}[\mathcal{W}_2^2(\nu_{g^*|S}, \nu_{h | S})] &= \mathbb{E}[\norm{T_S(g^*(\boldsymbol{X}, S)) - g^*(\boldsymbol{X}, S)}^2] \geq \inf_{h \in \mathcal{H}} \mathbb{E}[\norm{h(\boldsymbol{X}, S) - g^*(\boldsymbol{X}, S)}^2]\enspace,
%\end{align*}
%Recall that the excess risk is defined as $\mathcal{E}(g) = \mathcal{R}(g) - \mathcal{R}^*$, with $\mathcal{R}^*$ the risk of the optimal predictor. We can then combine to obtain the first part of Theorem 3.2 (and at the same time, Proposition 2.5). 
%\begin{equation}
%    \mathcal{E}(\mathcal{H}^0) = \mathcal{R}(\mathcal{H}^0) - \mathcal{R}^* = \inf_{g\theta \in \mathcal{H}}\sum p_s \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{h})
%\end{equation}
%which concludes the proof.
%\end{proof}

Considering Lemma~\ref{lem:ERisk}, as $\mathcal{G}^0$ and $\mathcal{G}^0_\Theta$ represent the subclass of DP-fair regressors, we can easily deduce Eq.~\eqref{eq:FairExcessRisk} and Eq.~\eqref{eq:ExcessRiskParam}:
    \begin{equation*}
        \mathcal{E}(\mathcal{G}^0) = \inf_{g \in \mathcal{G}}\sum_{s\in\mathcal{S}}p_s \mathcal{W}_2^2\left(\nu_{g^*|s}, \nu_{g}\right)
    \quad \text{ and }\quad 
        \mathcal{E}(\mathcal{G}_\Theta^0) = \inf_{g_\theta \in \mathcal{G}_\Theta}\sum_{s\in\mathcal{S}}p_s \mathcal{W}_2^2\left(\nu_{g^*|s}, \nu_{g_\theta}\right)\enspace.
    \end{equation*}


\subsection{Parametric Fair Predictor}\label{subappx:main}

\begin{proof}[\textbf{Proof of Proposition 3.1.}]

Following Eq.~\eqref{eq:ExcessRiskParam}, let $g_\theta \in \mathcal{G}_\Theta$ and applying the Minkowski inequality, we have
        \begin{align*}
            \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g_\theta}) \leq 2 \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g^{(0)*}}) + 2 \mathcal{W}_2^2(\nu_{g^{(0)*}}, \nu_{g_\theta}) \quad \text{for all }s\in\mathcal{S} \enspace.
        \end{align*}
        Hence, if we denote $g_\theta^*$ a minimizer of the r.h.s. of the above equation, then
        \begin{align*}
            \inf_{g_\theta \in \mathcal{G}_\Theta} \sum_{s\in\mathcal{S}} p_s \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g_\theta}) \leq 
            \sum_{s\in\mathcal{S}} p_s \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g_\theta^*}) \leq 2\sum_{s\in\mathcal{S}} p_s \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g^{(0)*}}) + 2 \mathcal{W}_2^2(\nu_{g^{(0)*}}, \nu_{g_\theta^*})\enspace,
        \end{align*}
        which implies:
        \begin{equation*}
            \mathcal{E}(\mathcal{G}^0) \leq \mathcal{E}(\mathcal{G}_\Theta^0) \leq 2\left(\mathcal{E}(\mathcal{G}^0) + \inf_{g_\theta \in \mathcal{G}_\Theta} \mathcal{W}_2^2(\nu_{g^{(0)*}}, \nu_{g_\theta})\right)\enspace.
        \end{equation*}

Finally, since $\mathbb{E}[g^*] = \mathbb{E}[g^{(0)*}]$, we derive the bounds on the following budget deviation $\mathcal{D}(g_\theta) = \mathbb{E}[g_\theta - g^{(0)*}]$ instead and we can infer the following upper bound
        \begin{align*}
            \mathcal{D}(g_\theta)^2 \leq \mathbb{E}[(g_\theta - g^{(0)*})^2] \leq \mathcal{W}_2^2 (\nu_{g^{(0)*}}, \nu_{g_\theta}), \quad \text{for all } g_\theta \in \mathcal{G}_\Theta\enspace,
        \end{align*}
        where we used Jensen's inequality on the left side inequality. In words this means that %within $\mathcal{G}_\Theta^0$, 
        $\mathcal{D}(g_\theta)^2$ is controlled by the distributional distance between $g_\theta$ and $g^{(0)*}$. Therefore, within $\mathcal{G}_\Theta$, 
 $g_\theta^{*}$ corresponds to the best solution for budget stability in terms of the $L_2$ norm. Additionally, replacing $g_\theta$ with $g_\theta^{(0)*}$ in the inequality above concludes the proof.
 %the inequality for $\norm{D(\Tilde{h}^{(\varepsilon)})}^2$ is therefore quite straightforward.
\end{proof}

\subsection{Extension to Approximate Fairness}
\label{subappx:approx}

Before going into the main proposition, let us present and prove the following lemma:
\begin{lem}[Risk-unfairness trade-off for interpolation cases]
    For any interpolated predictor of the form:
    $$
    g^{(\varepsilon)}(\boldsymbol{X}, S) = (1-\varepsilon)\cdot g(\boldsymbol{X}, S) + \varepsilon \cdot g^{*}(\boldsymbol{X}, S)
    $$
    with $g\in\mathcal{G}$, we have
    $$
    \mathcal{R}(g^{(\varepsilon)}) = (1-\varepsilon)^2 \cdot \mathcal{R}(g)\quad \text{ and }\quad \mathcal{U}(g^{\varepsilon}) = \varepsilon \cdot \mathcal{U}(g^*)\enspace.
    $$
\end{lem}
\begin{proof}
    For any $g \in \mathcal{G}$, the associated $g^{(\varepsilon)}$ verifies:
        \begin{align*}
            \mathcal{R}(g^{(\varepsilon)}) &= \mathbb{E}[((1-\varepsilon)\cdot g(\boldsymbol{X}, S) + \varepsilon\cdot g^* (\boldsymbol{X}, S) - g^*(\boldsymbol{X}, S))^2] \\
            &=
            \mathbb{E}[((1-\varepsilon)\cdot(g(\boldsymbol{X}, S) - g^*(\boldsymbol{X}, S)))^2] \\
            &= (1-\varepsilon)^2\cdot \mathcal{R}(g) \\
    \mathcal{U}(g^{\varepsilon}) &= \max_{s\in \mathcal{S}}\mathcal{W}_1(\nu_{g^{(\varepsilon)}{|s}}, \nu_{g^{(\varepsilon)}}) = \max_{s\in \mathcal{S}} \varepsilon\mathcal{W}_1(\nu_{g^*|s}, \nu_{g^*}) + 0 = \varepsilon \times \mathcal{U}(g^*)
        \end{align*}
\end{proof}

Thus, through this Lemma we have demonstrated Lemma~\ref{lem:RiskUnf} and Proposition~\ref{prop:ParamFairPredictorApprox}-i).

\begin{proof}[\textbf{Proof of Proposition~\ref{prop:ParamFairPredictorApprox}.}]
We divide the proof into parts according to the three sub-points i), ii) and iii):
    \begin{enumerate}
        \item[i)] {proven above.
        }
        \item[ii)]{
        To derive the approximate parametric fairness, we first define $g^{(\varepsilon)*}$ and $\Tilde{h}^{(\varepsilon)}$ as the solutions to the two following optimization problems:
        \begin{align*}
            \mathcal{E}(\mathcal{H}^\varepsilon) & = \sum_{s\in\mathcal{S}} p_s \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{\Tilde{h}^{(\varepsilon)}| s}) \\
            \mathcal{E}(\mathcal{G}^\varepsilon) & = \sum_{s\in\mathcal{S}} p_s \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g^{(\varepsilon)*}|s}) = (1-\varepsilon)^2 \sum_{s\in\mathcal{S}} p_s \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g^{(0)*}})
        \end{align*}
        Then, by the definition of $\mathcal{G}^\varepsilon$ and $\mathcal{H}^\varepsilon$, there exists $g^{(0)*}$ and $g^{(0)*}_\theta$ such that:
        \begin{align*}
            g^{(\varepsilon)*}(\boldsymbol{X}, S) & = (1-\varepsilon)\cdot g^{(0)*}(\boldsymbol{X}, S) + \varepsilon\cdot g^*(\boldsymbol{X}, S) \enspace,\\
            \Tilde{h}^{(\varepsilon)}(\boldsymbol{X}, S) &= (1-\varepsilon)\cdot g_\theta^{(0)*}(\boldsymbol{X}, S) + \varepsilon\cdot g^*(\boldsymbol{X}, S) \enspace.
        \end{align*}
        Further $g^{(0)*}$ corresponds to the Wasserstein barycenter defined in proposition 2.5 and $g_\theta^{(0)*}$ corresponds to the $\min$ specified in i). Conversely, we also have:
        \begin{align*}
            \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{h^{(\varepsilon)}|s}) \leq 2 \mathcal{W}_2^2(\nu_{g^*|s}, \nu_{g^{(\varepsilon)*}|s}) + 2\mathcal{W}_2^2(\nu_{g^{(\varepsilon)*}|s}, \nu_{h^{(\varepsilon)}|s})\enspace.
        \end{align*}
        
        Together with the fact that $\mathcal{E}(\mathcal{G}^{\varepsilon}) = (1-\varepsilon)^2\mathcal{E}(\mathcal{G}^0)$ we recover the main statement:
        
        \begin{align*}
            0 \leq \mathcal{E}(\mathcal{G}^\varepsilon) \leq \mathcal{E}(\mathcal{H}^\varepsilon) \leq 2(1-\varepsilon)^2\big(\mathcal{E}(\mathcal{G}^0) + \inf_{g_\theta \in \mathcal{G}_\Theta} \mathcal{W}_2^2(\nu_{g^{(0)*}}, \nu_{g_\theta}) \big)\enspace.
        \end{align*}
        }
        \item[iii)] 
        Since $\mathbb{E}[g^*] = \mathbb{E}[g^{(0)*}]$, it becomes apparent that for any $\varepsilon\in[0, 1]$, the equality $\mathbb{E}[g^*] =\mathbb{E}[g^{(\varepsilon)*}]$ holds true. Further, using Jensen's inequality, we derive straightforwardly the upper-bound on the squared budget deviation:
        \begin{align*}
            \mathcal{D}(h^{(\varepsilon)} )^2 = \mathbb{E}(h^{(\varepsilon)} - g^{(\varepsilon)*})^2 \leq \mathbb{E}[(h^{(\varepsilon)}  - g^{(\varepsilon)*})^2] \leq \mathcal{W}_2^2 (\nu_{g^{(\varepsilon)*}}, \nu_{h^{(\varepsilon)} }), \quad \text{for all } h^{(\varepsilon)}  \in \mathcal{H}^{(\varepsilon)}\enspace.
        \end{align*}
        Finally, replacing $h^{(\varepsilon)}$ with $\Tilde{h}^{(\varepsilon)}$ in the inequality above concludes the proof.
 %the inequality for $\norm{D(\Tilde{h}^{(\varepsilon)})}^2$ is therefore quite straightforward.
    \end{enumerate}
\end{proof}


\subsection{Statistical Guarantees}\label{subappx:cvg}

First, we establish the estimation guarantee before delving into the fairness guarantee. Note that we have adapted the estimation guarantee sequentially from \cite{gouic2020projection}, and \cite{bernton2019parameter} to account for the parametric framework. 

First, recall that throughout the paper, Assumption~\ref{assu:general} must hold.

\paragraph{Estimation Guarantee for $\varepsilon = 0$}

We denote $\Hat{\nu}_g$ as the empirical measure of $\nu_g$. To outline our statistical guarantees, let us present all the necessary assumptions:


%To this end, we require additional assumptions on $g^{(0)*}$ and its empirical counterpart $\Hat{g}^{(0)}$.
\begin{assu}[Smoothness \& Bound assumption]\label{assu:Lips}
    We assume that $(\Hat{g}(\cdot, s) )_{s\in\mathcal{S}}$ are uniformly Lipschitz and the estimator $\Hat{g}$ is bounded.
\end{assu}
With this assumption, we are then able to derive the following estimation guarantee for $\Hat{g}^{(0)}$, estimator of $g^{(0)*}$.
\begin{lem}[adapted from \cite{gouic2020projection} Thm.~8]
\label{lem:gouic}
    Under Assumption~\ref{assu:Lips}, and, as $n\to \infty$, assuming the following $L_2$-consistency
$$
\mathbb{E}[(g^*(\boldsymbol{X}, S) - \hat{g}(\boldsymbol{X}, S))^2] \to 0\enspace,
$$
we have both,
$$
\mathcal{W}_2^2 (\Hat{\nu}_{\hat{g}|s}, \nu_{g^{*}|s}) \to 0 \quad \text{and}\quad \mathcal{W}_2^2 (\Hat{\nu}_{\hat{g}^{(0)}|s}, \nu_{g^{(0)*}}) \to 0\quad\text{a.s.}
$$  
%$$
%\mathcal{W}_2(\nu_{g^{(0)*}}, \Hat{\nu}_{\Hat{g}^{(0)}}) \to 0 \quad a.s \enspace.
%$$
\end{lem}

Let us now consider the estimation guarantees in the parametric framework for $\Hat{g}_\theta$, estimator of $\Tilde{g}_\theta$. The Minimum Wasserstein Estimator (MWE) can be computationally intractable, especially in settings where simulating data from the model is possible but evaluating its density is not. In such cases, the Minimum Expected Wasserstein Estimator (MEWE) may offer a more computationally convenient alternative, where the expectation is replaced with a Monte Carlo approximation. Further, given that we explicitly want to sample from a parametric distribution, this approach is particularly attractive (see~\cite{bernton2019parameter} for more details). For simplicity, since it has been shown that MEWE converges to MWE and since in practice we have chosen a sufficiently large Monte Carlo sample to generate $\Hat{g}_\theta$, we omit the assumptions associated with Monte Carlo approximation.

\begin{assu}
\label{assu:mewe}
%Assume that the set of parameters $\Theta$ has $\norm{\cdot}_\Theta$ as a norm. 
The assumptions are as follows:
    \begin{enumerate}
        \item $\mathcal{G}_\Theta$ is a family of continuous distributions.
        \item The map $\theta \mapsto \nu_{g_\theta}$ is continuous.
        %\item For some $\alpha > 0$, the set $B^*(\alpha) = \{ \theta \in \Theta: \mathcal{W}_2(\nu_{g^{(0)*}}, \nu_{g_\theta}) \leq \inf_{\theta\in\Theta}\mathcal{W}_2(\nu_{g^{(0)*}}, \nu_{g_\theta}) + \alpha \}$ is bounded.
        \item For some $\alpha > 0$, the set $B_n(\alpha) = \{ \theta \in \Theta: \mathcal{W}_2(\Hat{\nu}_{\Hat{g}^{(0)}}, \nu_{g_\theta}) \leq \inf_{g_\theta\in\mathcal{G}_\Theta}\mathcal{W}_2(\Hat{\nu}_{\Hat{g}^{(0)}}, \nu_{g_\theta}) + \alpha \}$ is bounded.
        %\item For some $\alpha > 0$, the set $B_{*}(\alpha) = \{ ... \}$
        %\item For any $m\geq 1$ if $\norm{\Hat{\theta} -\theta}_\Theta \to 0$, then $\mathcal{W}_2(\Hat{\nu}_{\Hat{g}_\theta}, ...) ...$ as $n\to\infty$.
        %\item ...
        %\item (2.8.) For some $\alpha > 0$, the set $B_n(\alpha) = \{ \theta \in \Theta: \mathcal{W}_2(\Hat{\nu}_{\Hat{g}_\theta}, \nu_{g_\theta}) \leq \inf_{\theta\in\Theta}\mathcal{W}_2(\Hat{\nu}_{\Hat{g}_\theta}, \nu_{g_\theta}) + \alpha \}$ is bounded.
    \end{enumerate}
\end{assu}

\begin{lem}[Existence and consistency, adapted from \cite{bernton2019parameter} Thm.~2.1 and Thm.~2.4]
\label{lem:bernton}
    Under Assumption~\ref{assu:Lips} and Assumption~\ref{assu:mewe}, as $n\to\infty$,
    $$
    \inf_{\Hat{g}_\theta\in\mathcal{G}_\Theta} \mathcal{W}_2(\Hat{\nu}_{\Hat{g}^{(0)}}, \Hat{\nu}_{\Hat{g}_{\theta}}) \to \inf_{g_\theta\in\mathcal{G}_\Theta}\mathcal{W}_2(\nu_{g^{(0)*}}, \nu_{g_\theta})\quad a.s.\enspace,
    $$
    and \textit{a.s.} for a large enough sample, the sets $\argmin{}_{\Hat{g}_\theta\in\mathcal{G}_\Theta} \mathcal{W}_2(\Hat{\nu}_{\Hat{g}^{(0)}}, \Hat{\nu}_{\Hat{g}_{\theta}})$ are non-empty and form a bounded sequence with
    $$
    \lim \sup_{n\to\infty} \argmin{\Hat{g}_\theta\in\mathcal{G}_\Theta} \mathcal{W}_2(\Hat{\nu}_{\Hat{g}^{(0)}}, \Hat{\nu}_{\Hat{g}_{\theta}}) \subset \argmin{g_\theta\in\mathcal{G}_\Theta}\mathcal{W}_2(\nu_{g^{(0)*}}, \nu_{g_\theta})\enspace.
    $$
\end{lem}

%\mathcal{W}_2^2 (\Hat{\nu}_{\hat{g}_{|s}}, \nu_{g^*_{|s}})    &\leq 2 \mathbb{E}[\norm{g^*(\boldsymbol{X}, S) - \hat{g}(\boldsymbol{X}, S)}^2] + 2 L^2 \mathbb{E}[\norm{\boldsymbol{X} - T_x(\boldsymbol{X}, S)}^2] + 8M\mathbb{P}(T_s(\boldsymbol{X}, S)\neq S) \\ & \leq 2 \mathbb{E}[\norm{g^*(\boldsymbol{X}, S) - \hat{g}(\boldsymbol{X}, S)}^2] + (2L^2 + 8M)\mathcal{W}_2^2( \mathbb{P}_{(\boldsymbol{X}, S)}, \Hat{\mathbb{P}}_{(\boldsymbol{X}, S)})\enspace,
    %\end{align*}
%which concludes the first part of the proof.

%\fran{Q: Si this enough ?}
%We recall that 
%$$
%\Tilde{g}_\theta = \argmin{g_\theta\in\mathcal{G}_\Theta}\mathcal{W}_2(\nu_{g^{(0)*}}, \nu_{g_\theta})\enspace.
%$$
%Following the above results we can now prove the convergence of the parametric fair estimator $\Hat{\nu}_{\Hat{g}_\theta}$ to $\nu_{\Tilde{g}_\theta}$. %To do so, as $\n\to +\infty$, we assume that
%$$
%\mathbb{E}[(g^*(\boldsymbol{X}, S) - \hat{g}(\boldsymbol{X}, S))^2] \to 0\enspace.
%$$
%Then, from the above inequality (first part of the proof) and the Wasserstein barycenter setup, we have both,
%$$
%\mathcal{W}_2^2 (\Hat{\nu}_{\hat{g}|s}, \nu_{g^{*}|s}) \to 0 \quad \text{and}\quad \mathcal{W}_2^2 (\Hat{\nu}_{\hat{g}^{(0)}|s}, \nu_{g^{(0)*}}) \to 0\quad\text{a.s.}
%$$
%Indeed, from the triangle inequality, we have
%$$
%0 \leq \mathcal{W}_2 (\Hat{\nu}_{\hat{g}_\theta}, \nu_{\Tilde{g}_\theta}) \leq \mathcal{W}_2 (\Hat{\nu}_{\hat{g}_\theta}, ...) + \mathcal{W}_2 (..., \nu_{\Tilde{g}_\theta})
%$$
Note that the detailed rate of convergence, under stronger assumptions, can also be found in \cite{bernton2019parameter}.



%{\color{green} --> problem, c'était avec \cite{bernton2019parameter}, mais plutot $\mathcal{W}_2(\nu_{\hat{g}_\theta}, \nu_{g_\theta})$}
%{\color{blue} --> sorry my bad, c'est bien de $\mathcal{W}_2 (\Hat{\nu}_{\Hat{g}_\theta^{(0)}}, \nu_{g_\theta^{(0)*}})$}
%... which implies the convergence of $\Hat{\nu}_{\hat{g}_\theta^{(0)}|s}$.

\paragraph{Estimation Guarantee for $\varepsilon \geq 0$ (Corollary~\ref{coro:estimation})}

Since, with the geodesic interpolation, we have
$$
\Tilde{h}^{(\varepsilon)}(\boldsymbol{X}, S) = (1-\varepsilon)\cdot \Tilde{g}_\theta(\boldsymbol{X}, S) + \varepsilon \cdot g^{*}(\boldsymbol{X}, S)\enspace,
$$
and 
$$
\hat{h}^{(\varepsilon)}(\boldsymbol{X}, S) = (1-\varepsilon)\cdot \Hat{g}_\theta(\boldsymbol{X}, S) + \varepsilon \cdot \Hat{g}(\boldsymbol{X}, S)\enspace,
$$
by the above results (Lemma~\ref{lem:gouic} and Lemma~\ref{lem:bernton}), as $n\to+\infty$, we have directly
$$
\mathcal{W}_2\left(\Hat{\nu}_{\hat{h}^{(\varepsilon)}}, \nu_{\Tilde{h}^{(\varepsilon)}}\right) \to 0\quad a.s\enspace.
$$

%\fran{à re-vérifier: $\Tilde{g}_\theta$ fair ?}
\paragraph{Fairness Guarantee (Corollary~\ref{coro:fairness})} Recall Assumptions \ref{assu:Lips}-\ref{assu:mewe} and the above $L_2$-consistency of $\Hat{g}$.
Given $\varepsilon \in[0, 1]$, we observe asymptotic fairness with $\varepsilon$-RI. Indeed, since by construction $\Tilde{g}_\theta$ is independent to $S$ and by applying triangle inequality, we have for all $s\in\mathcal{S}$,
\begin{align*}
\mathcal{W}_1\left(\hat{\nu}_{\hat{h}^{(\varepsilon)}|s}, \hat{\nu}_{\hat{h}^{(\varepsilon)}}\right) &\leq \mathcal{W}_1\left(\hat{\nu}_{\hat{h}^{(\varepsilon)}|s}, \nu_{\Tilde{h}^{(\varepsilon)}|s}\right) + 
\mathcal{W}_1\left(\nu_{\Tilde{h}^{(\varepsilon)}|s}, \nu_{\Tilde{h}^{(\varepsilon)}}\right)+
\mathcal{W}_1\left(\nu_{\Tilde{h}^{(\varepsilon)}}, \hat{\nu}_{\hat{h}^{(\varepsilon)}}\right)\\
&\leq \varepsilon\times \mathcal{U}(g^*) + \mathcal{W}_1\left(\hat{\nu}_{\hat{h}^{(\varepsilon)}|s}, \nu_{\Tilde{h}^{(\varepsilon)}|s}\right) + \mathcal{W}_1\left(\nu_{\Tilde{h}^{(\varepsilon)}}, \hat{\nu}_{\hat{h}^{(\varepsilon)}}\right)\enspace,
\end{align*}
where the two right terms on the right side of the inequality tends towards zero. This convergence is achieved due to the fact that convergence in $\mathcal{W}_2$ implies convergence in $\mathcal{W}_1$.
%can use the fact that congervence in 2-Wasserstein distance implies convergence in 1-Wasserstein distance.

%\bibliography{biblio}

%\end{document}













==> tabs/tab_sims.tex <==
\begin{table}[htbp]
\footnotesize
\begin{center}
\def\arraystretch{1.55}%
\setlength\tabcolsep{1.8pt}
\resizebox{\columnwidth}{!}{%
%\begin{tabularx}{\columnwidth}{|x x x x|}
\begin{tabular}{|c c c c|}
\hline
  & \textbf{\textit{Uncorrected}} & \textbf{\textit{Standard}} & \textbf{\textit{Parametric}} \\
\hline
 & \multicolumn{3}{c|}{\textit{Classification - \texttt{Compas} - Normal }}\\
\cline{2-4}
Observed & 0.032 $\pm$ 0.023 & 0.026 $\pm$ 0.014 & 0.012 $\pm$ 0.007 \\
Latent & 0.111 $\pm$ 0.084 & 0.116 $\pm$ 0.086 & 0.045 $\pm$ 0.025\\
F1 & 0.221 $\pm$ 0.078 & 0.231 $\pm$ 0.080 & 0.227 $\pm$ 0.078\\
& \multicolumn{3}{c|}{\textit{Classification - \texttt{folktables} - Beta}}\\
\cline{2-4}
Observed & 0.586 $\pm$ 0.005 & 0.016 $\pm$ 0.007 & 0.038 $\pm$ 0.022 \\
Latent & 0.328 $\pm$ 0.004 & 0.213 $\pm$ 0.004 & 0.120 $\pm$ 0.002\\

F1, $\varepsilon$=0.00 & 0.538 $\pm$ 0.001 & 0.516 $\pm$ 0.004 & 0.513 $\pm$ 0.003\\
F1, $\varepsilon$=0.25 & 0.538 $\pm$  0.001& 0.519 $\pm$ 0.003 & 0.517 $\pm$ 0.003\\
F1, $\varepsilon$=0.50 & 0.538 $\pm$ 0.001& 0.528 $\pm$ 0.003 & 0.527 $\pm$ 0.003\\
F1, $\varepsilon$=0.75 & 0.538 $\pm$ 0.001& 0.535 $\pm$ 0.002 & 0.536 $\pm$ 0.002\\

%\hline
& \multicolumn{3}{c|}{\textit{Regression - \texttt{folktables} - Measurement Error}}\\
\cline{2-4}
MSE - 0\% & N/A & 0.553 $\pm$ 0.006 & 0.569 $\pm$ 0.007 \\
MSE - 25\% & N/A & 0.711 $\pm$ 0.007 & 0.709 $\pm$ 0.007 \\
MSE - 50\% & N/A & 1.873 $\pm$ 0.014 & 1.737 $\pm$ 0.016 \\
MSE - 75\% & N/A & 5.704 $\pm$ 0.027 & 4.764 $\pm$ 0.027 \\
\hline
%\hline
\end{tabular}
}
\end{center}
\label{tab:sims}
\caption{Results for simulations, indicated are means over the simulations with standard errors reported. Note that the \textit{Uncorrected} column for the folktables classification task stays constant across all $\varepsilon$ values as it is the basis of interpolation. }
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}


